iCAN: Instance-Centric Attention Network for Human-Object Interaction Detection

Recent years have witnessed rapid progress in detecting and recognizing individual object instances. To understand the situation in a scene, however, computers need to recognize how humans interact with surrounding objects. In this paper, we tackle the challenging task of detecting human-object interactions (HOI). Our core idea is that the appearance of a person or an object instance contains informative cues on which relevant parts of an image to attend to for facilitating interaction prediction. To exploit these cues, we propose an instance-centric attention module that learns to dynamically highlight regions in an image conditioned on the appearance of each instance. Such an attention-based network allows us to selectively aggregate features relevant for recognizing HOIs. We validate the efficacy of the proposed network on the Verb in COCO and HICO-DET datasets and show that our approach compares favorably with the state-of-the-arts.

==> fig/fig_ablation_time.tex <==
\begin{figure}[t]
    \centering
	{\includegraphics[width=1.0 \linewidth]{figure/VCOCO_ablation_time.png}}\hfill
    
\vspace{3mm}
\captionof{figure}{Comparison about mAP, inference time and the model size.}
\label{fig:time}
\end{figure}

==> fig/fig_att_H.tex <==
\begin{figure}[h]
\centering
\footnotesize
%\jbox{\textwidth}{0.3\textwidth}
%\includegraphics[width=1.0 \linewidth]{figure/detection.pdf}

\mpage{0.22}{\includegraphics[width=\linewidth]{figure_peak/new_008992_2014.png}}
\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_peak/new_3.png}}
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_peak/new_4.png}}
\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_peak/new_1.png}}
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_peak/new_2.png}}

\vspace{\figmargin}
\caption{\tb{Human-centric attention.} We crop $100\times 100$ patches centered at the peaks of the attentional maps generated by the two persons.
}
\vspace{\figbmargin}
\label{fig:att_H}
\end{figure}


% \mpage{0.23}{\includegraphics[width=\linewidth]{figure_att/007158_292463_aa.png}}
% \mpage{0.23}{\includegraphics[width=\linewidth]{figure_att/007158_292463_overlay_H.png}}\hfill
% \mpage{0.23}{\includegraphics[width=\linewidth]{figure_att/007368_292463_aa.png}}
% \mpage{0.23}{\includegraphics[width=\linewidth]{figure_att/007368_292463_overlay_H.png}}


% \mpage{0.23}{\scriptsize sit on chair; eat}\hfill
% \mpage{0.23}{\scriptsize Human-centric att.}\hfill
% \mpage{0.23}{\scriptsize sit on chair; eat}\hfill
% \mpage{0.23}{\scriptsize Human-centric att.}\hfill


==> fig/fig_error.tex <==
\begin{figure}[t]
    \centering
	{\includegraphics[width=1.0 \linewidth]{figure/Error_Analysis_bar.pdf}}\hfill
    
\vspace{\figmargin}
\captionof{figure}{
Distribution of the incorrect detections for each action class. \tb{`incorrect label'} refers to when the detected person is not doing this action. \tb{`bck'} indicates when the object detection branch totally fails to localize person (IoU with any ground truth person less than 0.1). \tb{`person misloc'} means when the object detection branch imperfectly localizes the person (regardless of related object). \tb{`object misloc'} refers to when the object detection branch imperfectly localizes the object (while successfully localizes the related person). \tb{`mis-grouping'} indicates when the person is successfully localized but the network fails to match the person to the correct related object.
\tb{`occlusion'} means we associate an object instance with a correct detected person, while the object is not annotated in the ground truth due to occlusions.
}
    \label{fig:error}
\end{figure}

==> fig/fig_failure.tex <==
\begin{figure}[t]
    \centering
    \hfill
	\mpage{0.18}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_1.png}}\hfill
	\mpage{0.09}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_5.png}}\hfill
    \mpage{0.18}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_2.png}}\hfill
    \mpage{0.18}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_3.png}}\hfill
    \mpage{0.18}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_4.png}}\hfill
    \mpage{0.09}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_1_6.png}}\hfill
    
    \mpage{0.34}{{\scriptsize snowboarding}}
    \mpage{0.10}{{\scriptsize catch frisbee}}\hfill
    \mpage{0.24}{{\scriptsize ride car}}\hfill
    \mpage{0.16}{{\scriptsize kick sports ball}}\hfill
    \mpage{0.08}{{\scriptsize eat pizza}}
    
    \hfill
	\mpage{0.22}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_2_1.png}}\hfill
	\mpage{0.17}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_2_2.png}}\hfill
    \mpage{0.17}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_2_3.png}}\hfill
    \mpage{0.17}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_2_4.png}}\hfill
    \mpage{0.17}{\includegraphics[width=1.0 \linewidth]{figure_detection/False_2_5.png}}\hfill

    \mpage{0.22}{{\scriptsize ride horse}}
    \mpage{0.17}{{\scriptsize surf surfboard}}
    \mpage{0.17}{{\scriptsize ride bike}}
    \mpage{0.17}{{\scriptsize surf surfboard}}
    \mpage{0.17}{{\scriptsize ride motorcycle}}
    
\vspace{\figmargin}
    \captionof{figure}{
    \textbf{Visualizations of the incorrect detections.} 
    First row: incorrect label. Second row: mis grouping (1st and 2nd) and object mis-localization (3rd to 5th).
    %
    Red box indicates the detected person, blue box means the (incorrect) detected object, green box shows the ground truth object annotation.
    }
    \label{fig:failure}
\end{figure}

==> fig/fig_motivation.tex <==
% Motivation 
\begin{figure}[t]
\centering
\hfill
\mpage{0.3}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_object.pdf}}\hfill
\mpage{0.22}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_scene.pdf}}\hfill
%\mpage{0.31}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_sp.pdf}} 
\begin{minipage}{0.45\linewidth}\centering
\mpage{0.46}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_sp_11.pdf}} 
\mpage{0.46}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_sp_12.pdf}} 
\mpage{0.4}{{\scriptsize \tb{\red{Human}} riding \tb{\blue{horse}}?}}
\mpage{0.4}{{\scriptsize No interaction!}}
\mpage{0.47}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_sp_21.pdf}}
\mpage{0.42}{\includegraphics[width=1.0 \linewidth]{figure/Motivation_sp_22.pdf}}
\mpage{0.54}{{\scriptsize \tb{\red{Human}} surfing \tb{\blue{surfboard}}?}}
\mpage{0.4}{{\scriptsize No interaction!}}
\end{minipage}\hfill

\mpage{0.3}{Interactee}\hfill
\mpage{0.22}{Context}\hfill
\mpage{0.45}{Spatial configuration}\hfill
\vspace{\figcapmargin}
\caption{\textbf{Importance of jointly considering object that the person is interacting with.} Left: Human-centric approaches infer the person's action through its appearance. Right: identifying the object they are interacting with reduces the ambiguity. \tb{Importance of contextual scene.} The information of the surround scenes provides important cues for recognizing the action performed by the person: person driving a horse drawn carriage. We introduce a context branch to capture such information to complement the appearance features focusing only on the human and object. \tb{Importance of spatial configuration.} Recognizing human-object interaction without considering spatial layout leads to plausible but incorrect predictions. Two illustrative examples demonstrate the difficulty of HOI detection based on appearance of human and object.}
\label{fig:motivation}
\end{figure}

==> fig/fig_result.tex <==
\begin{figure*}[t]
\centering
\footnotesize
%\jbox{\textwidth}{0.3\textwidth}
%\includegraphics[width=1.0 \linewidth]{figure/detection.pdf}

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/1_6.jpg}}\hfill
%\vspace{\figcapmargin}
\mpage{0.15}{\scriptsize surf       surfboard}\hfill
\mpage{0.15}{\scriptsize carry      suitcase}\hfill
\mpage{0.15}{\scriptsize ride       horse}\hfill
\mpage{0.15}{\scriptsize catch      frisbee}\hfill
\mpage{0.15}{\scriptsize skateboarding}\hfill
\mpage{0.15}{\scriptsize eat hot dog}\hfill
%\vspace{\figcapmargin}


\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/2_6.jpg}}\hfill
\mpage{0.15}{\scriptsize talk on cellphone}\hfill
\mpage{0.15}{\scriptsize hit with racket}\hfill
\mpage{0.15}{\scriptsize kick sports ball}\hfill
\mpage{0.15}{\scriptsize drink with cup}\hfill
\mpage{0.15}{\scriptsize work on laptop}\hfill
\mpage{0.15}{\scriptsize snowboarding}\hfill


%\vspace{\figcapmargin}
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/3_6.jpg}}\hfill
\mpage{0.15}{\scriptsize cut with   knife}\hfill
\mpage{0.15}{\scriptsize skiing        }\hfill
\mpage{0.15}{\scriptsize hold       umbrella}\hfill
\mpage{0.15}{\scriptsize lay in     bed}\hfill
\mpage{0.15}{\scriptsize cut        cake}\hfill
\mpage{0.15}{\scriptsize throw      Frisbee}\hfill



\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/4_6.jpg}}\hfill
\mpage{0.15}{\scriptsize read     book}\hfill
\mpage{0.15}{\scriptsize hit with bat}\hfill
\mpage{0.15}{\scriptsize hold     cup}\hfill
\mpage{0.15}{\scriptsize sit on   motorcycle}\hfill
\mpage{0.15}{\scriptsize throw    sports ball}\hfill
\mpage{0.15}{\scriptsize ride     elephant}\hfill


\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/5_6.jpg}}\hfill
\mpage{0.15}{ride   bicycle}\hfill
\mpage{0.15}{drink with cup}\hfill
\mpage{0.15}{surf surfboard}\hfill
\mpage{0.15}{work on laptop}\hfill
\mpage{0.15}{lay in bed}\hfill
\mpage{0.15}{surf surfboard}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/6_6.jpg}}\hfill

\mpage{0.15}{work on laptop}\hfill
\mpage{0.15}{lay in couch}\hfill
\mpage{0.15}{kick sports ball}\hfill
\mpage{0.15}{skiing}\hfill
\mpage{0.15}{sit on horse}\hfill
\mpage{0.15}{drink with cup}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/7_6.jpg}}\hfill

\mpage{0.15}{hit with tennis racket}\hfill
\mpage{0.15}{eat with spoon}\hfill
\mpage{0.15}{jump skateboard}\hfill
\mpage{0.15}{cut with knife}\hfill
\mpage{0.15}{read book}\hfill
\mpage{0.15}{carry handbag}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_1.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_2.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_3.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_4.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_5.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection/8_6.jpg}}\hfill
\mpage{0.15}{cut with knife}\hfill
\mpage{0.15}{cut with scissor}\hfill
\mpage{0.15}{read book}\hfill
\mpage{0.15}{hit with baseball bat}\hfill
\mpage{0.15}{jump skateboard}\hfill
\mpage{0.15}{eat with fork}\hfill


\vspace{\figmargin}
\caption{\textbf{Detection results on V-COCO $\emph{test}$ set.} 
Our model can detect various forms of human-object interactions in everyday photos.
}
\label{fig:result}
\end{figure*}

==> fig/fig_result_HICO.tex <==
\begin{figure*}[t]
\centering
\footnotesize
%\jbox{\textwidth}{0.3\textwidth}
%\includegraphics[width=1.0 \linewidth]{figure/detection.pdf}

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hold_HICO_test2015_00007461.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/imspect_HICO_test2015_00005316.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/jump_HICO_test2015_00004493.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/race_HICO_test2015_00007750.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/turn_HICO_test2015_00005975.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/straddle_HICO_test2015_00008105.jpg}}\hfill

\mpage{0.15}{\scriptsize hold       motorcycle}\hfill
\mpage{0.15}{\scriptsize inspect       motorcycle}\hfill
\mpage{0.15}{\scriptsize jump       motorcycle}\hfill
\mpage{0.15}{\scriptsize race       motorcycle}\hfill
\mpage{0.15}{\scriptsize turn       motorcycle}\hfill
\mpage{0.15}{\scriptsize straddle   motor.}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/feed_HICO_test2015_00008897.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hose_test2015_00004915.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/kiss_HICO_test2015_00001938.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/pet_HICO_test2015_00002340.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/ride_HICO_test2015_00000469.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/walk_HICO_test2015_00004671.jpg}}\hfill

\mpage{0.15}{\scriptsize feed       elephant}\hfill
\mpage{0.15}{\scriptsize hose       elephant}\hfill
\mpage{0.15}{\scriptsize kiss       elephant}\hfill
\mpage{0.15}{\scriptsize pet       elephant}\hfill
\mpage{0.15}{\scriptsize ride       elephant}\hfill
\mpage{0.15}{\scriptsize walk       elephant}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/siton_HICO_test2015_00005683.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/wash_HICO_test2015_00003318.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/standon_HICO_test2015_00000333.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/drive_HICO_test2015_00009099.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/repair_HICO_test2015_00006558.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/row_HICO_test2015_00008418.jpg}}\hfill

\mpage{0.15}{\scriptsize sit on boat}\hfill
\mpage{0.15}{\scriptsize wash   boat}\hfill
\mpage{0.15}{\scriptsize stand on boat}\hfill
\mpage{0.15}{\scriptsize drive boat}\hfill
\mpage{0.15}{\scriptsize repair boat}\hfill
\mpage{0.15}{\scriptsize row boat}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/pet_HICO_test2015_00009227.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/walk_HICO_test2015_00009213.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/wash_HICO_test2015_00007600.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/kiss_HICO_test2015_00004193.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/dry_HICO_test2015_00007559.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/carry_HICO_test2015_00001121.jpg}}\hfill

\mpage{0.15}{\scriptsize pet dog}\hfill
\mpage{0.15}{\scriptsize walk   dog}\hfill
\mpage{0.15}{\scriptsize wash dog}\hfill
\mpage{0.15}{\scriptsize kiss dog}\hfill
\mpage{0.15}{\scriptsize dry dog}\hfill
\mpage{0.15}{\scriptsize carry dog}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/catch_HICO_test2015_00007239.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/throw_HICO_test2015_00008670.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/kick_HICO_test2015_00009555.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hold_HICO_test2015_00005519.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hit_HICO_test2015_00003459.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/dribble_HICO_test2015_00000272.jpg}}\hfill

\mpage{0.15}{\scriptsize catch       sports ball}\hfill
\mpage{0.15}{\scriptsize throw       sports ball}\hfill
\mpage{0.15}{\scriptsize kick       sports ball}\hfill
\mpage{0.15}{\scriptsize hold       sports ball}\hfill
\mpage{0.15}{\scriptsize hit       sports ball}\hfill
\mpage{0.15}{\scriptsize dribble sports ball}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/blow_HICO_test2015_00000148.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/carry_HICO_test2015_00006130.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/eat_HICO_test2015_00006802.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/make_HICO_test2015_00003351.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/light_HICO_test2015_00003673.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hold_HICO_test2015_00009402.jpg}}\hfill

\mpage{0.15}{\scriptsize blow       cake}\hfill
\mpage{0.15}{\scriptsize carry       cake}\hfill
\mpage{0.15}{\scriptsize eat       cake}\hfill
\mpage{0.15}{\scriptsize make       cake}\hfill
\mpage{0.15}{\scriptsize light       cake}\hfill
\mpage{0.15}{\scriptsize hold        cake}\hfill

\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/peel_HICO_test2015_00000250.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hold_HICO_test2015_00009493.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/cut_HICO_test2015_00001684.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/inspect_HICO_test2015_00006400.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/squeeze_HICO_test2015_00002314.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/wash_HICO_test2015_00009725.jpg}}\hfill

\mpage{0.15}{\scriptsize peel       orange}\hfill
\mpage{0.15}{\scriptsize hold        orange}\hfill
\mpage{0.15}{\scriptsize cut       orange}\hfill
\mpage{0.15}{\scriptsize inspect       orange}\hfill
\mpage{0.15}{\scriptsize squeeze       orange}\hfill
\mpage{0.15}{\scriptsize wash orange}\hfill


\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/hold_HICO_test2015_00003036.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/carry_HICO_test2015_00009148.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/drink_HICO_test2015_00002374.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/inspect_HICO_test2015_00008112.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/lick_HICO_test2015_00008986.jpg}}\hfill
\mpage{0.15}{\includegraphics[width=\linewidth]{figure_detection_HICO/pour_HICO_test2015_00000339.jpg}}\hfill

\mpage{0.15}{\scriptsize hold bottle}\hfill
\mpage{0.15}{\scriptsize carry   bottle}\hfill
\mpage{0.15}{\scriptsize drink bottle}\hfill
\mpage{0.15}{\scriptsize inspect bottle}\hfill
\mpage{0.15}{\scriptsize lick bottle}\hfill
\mpage{0.15}{\scriptsize pour bottle}\hfill

\vspace{\figmargin}
\caption{\textbf{Detection results on HICO-DET $\emph{test}$ set.}}
\label{fig:result_HICO}
\end{figure*}

==> method.tex <==
% \section{Framework}
% \label{sec:method}

% % Outline.
% In this section, we describe individual components of our Instance-centric Attention Network as shown in \figref{overview}. We outline the details of the three main branches for feature extraction: the human branch~(\secref{human}), the object branch~(\secref{object}), and the spatial configuration branch~(\secref{spatial}).

% \subsection{Instance-centric Module}
% \label{sec:instance}
% For each bounding box $b_h$/$b_o$ detected from off-the-shelf Faster R-CNN, we crop the feature map using the instance bounding box and resize to it to $7 \times 7$.
% %
% Then the instance feature is flattened and passed into 2 fully connected layers (with RELU \cite{Nair-ICML-RELU}) to yield an attention parameter vector, $b$.  
% %
% % How attention map is computed.
% Given the vector $b$ and the plain feature map, we compute an attention map over all $n$ spatial locations by taking the inner product of $b$ and the plain feature map at each spatial location, followed by a softmax layer.
% %
% % How instance-centric feature is generated.
% Then this normalized attention map is used for attentional pooling and contributes to instance-centric contextual feature.
% %
% The intuition behind is, we try to capture the compatibility between the human feature and global feature. That is, the attention map should have a high score locally if that region is informative and contains relevant contextual information for recognition.
% % 
% The purpose of this branch is to detect actions that do not involve any objects, \eg, walk, smile.

% \subsection{Human Branch}
% \label{sec:human}
% % Implementation details.
% For each human box $b_h$ detected from off-the-shelf Faster R-CNN, in human branch we crop the feature map using the human bounding box and resize to it to $7 \times 7$.
% %
% Then the human feature is flattened and passed into 2 fully connected layers (with RELU \cite{Nair-ICML-RELU}) to yield an attention parameter vector, $b$.  
% %
% % How attention map is computed.
% Given the vector $b$ and the plain feature map, we compute an attention map over all $n$ spatial locations by taking the inner product of $b$ and the plain feature map at each spatial location, followed by a softmax layer.
% %
% % How instance-centric feature is generated.
% Then this normalized attention map is used for attentional pooling and contributes to human-centric contextual feature.
% %
% % How to predict the action.
% The original human feature is passed through res5 block followed by an average pooling layer, then concatenated with the human-centric contextual feature, and passed into two fully-connected layers to predict the action score $s^a_h$. 
% %
% The intuition behind is, we try to capture the compatibility between the human feature and global feature. That is, the attention map should have a high score locally if that region is informative and contains relevant contextual information for recognition. \chen{Redundant. Move ahead.}
% % 
% The purpose of this branch is to detect actions that do not involve any objects, \eg, walk, smile.

% \subsection{Object Branch}
% \label{sec:object}
% %
% The object branch follows the same design, except the input is the object box $b_o$. The output of the last fully-connected layer (A-dimensional vectors of logit) is added together with the one from the human branch, and passed through a sigmoid activation layer to yield action score $s^a_{h,o}$. 

% \subsection{Spatial Configuration Branch}
% \label{sec:spatial}
% %
% % Why sp is important.
% While the human and object appearance features contain discriminative cues for recognizing the interaction, using appearance features alone often are not sufficient to resolve ambiguity, particularly when multiple persons and objects present in the scene.
% %
% %\figref{motivation} shows two examples to highlight the importance of considering spatial configuration.
% %
% % How to construct sp feature.
% To represent the spatial configuration,we adopt the two-channel binary image to characterize the interaction patterns~\cite{Chao-WACV-HOI}. Specifically, we regard the union of these two boxes as the reference box and construct the binary image within it. The aspect ratio is kept the size by resizing the longest side of the reference box to a fix length and padding zeros on both sides of the shorter side. The first channel has value 1 within human bounding box, and value 0 elsewhere; the second channel has value 1 within object bounding box, and value 0 elsewhere. 
% %
% % How to combine spatial and appearance feature together.
% We then use a CNN to extract features from this 2-channel binary image. We vectorize the activations and concatenate this spatial features with the human appearance feature for interaction recognition.
% %
% The feature is passed into two fully-connected layers to predict the action score $s^a_{sp}$. We multiply $s^a_{sp}$ and $s^a_{h,o}$ for the final prediction.

% %\subsection{Joint Branch}
% %\label{sec:interaction}


% \subsection{Multi-task Training}
% \label{sec:multitask}
% % What is the training loss.
% All the branches are trained jointly.
% %
% Our overall loss function is the summation of the action classification loss for
% (1) the human branch, and
% (2) the object branch, and
% (3) the spatial configuration branch
% %
% % How we augment the training data.
% To augment the positive training data, we jitter the human box and object box in the ground truth triplet to simulate additional 15 positive training triplets.
% %
% % How we construct Negative training data.
% We construct negative training examples by pairing all the Faster R-CNN detected humans and objects that are not in the ground truth.
% %
% The loss for both human and object branch is only computed on the 16 positive triplets. The loss for the spatial configuration branch is computed on the 16 positive triplets and negative triplets.

% \subsection{Efficient Inference}
% \label{sec:inference}
% %
% During inference, we predict the triplets in a cascade fashion. 
% % 
% % How do we generate object detections.
% First, we detect all the object instances in the image using the off-the-shelf Faster R-CNN. We maintain human boxes with scores $s_o$ higher than 0.8 and object boxes with scores $s_h$ higher than 0.4. We then apply NMS with an IoU threshold of 0.3 on the detected boxes.
% %
% % Inference procedure and complexity
% We compute the logit for the action classification head of the human branch for each box $b_h$ and the logit for the action classification head of the object branch for each box $b_o$. This step has a complexity of $O(n)$. Then we compute the logit for the action classification head of the spatial configuration branch for each box pair $b_h$ and $b_o$, and pass it through a sigmoid. Finally, to get scores $s^a_{h,o}$, the human branch logit and the object branch logit are summed and passed through a sigmoid for each pair, and is multiplied with the spatial configuration branch score. This step has a complexity of $O(n^2)$.

% % Special case: actions that have no objects
% To take care of the action that has no interaction with objects, we apply the human branch to all detected objects that were classified as human. For each action $a$ and detected human box $b_h$, we compute $s^a_h$, the score assigned to action $a$ by only considering human appearance. 



% %%%%%%%%%%
% %\subsection{Interaction Branch}
% %\label{sec:interaction}
% %
% %For each object box $b_o$, following the same procedure, we can extracts its appearance features from $b_o$ with RoIPooling. 
% %
% %In this branch, we concatenate appearance features of human and objects, the spatial features from the spatial configuration branch as well as contextual feature.
% %
% %We then feed this feature into fully-connected layers and predict an action score $s^a_{h,o}$.

% %Our method effectively leverage the both the human and object appearance in a \emph{early fusion} manner (as opposed to the \emph{late fusion} that fuse the prediction scores after the predictions are made from individual features).
% %
% %In the context of human-object interaction, performing early fusion is important because the action is closely related not only to the human appearance but also the object the person is interacting with.
% %
% %For example, we need to see a person and a horse to infer whether the action of the person is \textit{ride}, \textit{look} or \textit{stand} (no interaction). 
% %
% %In addition, the spatial features encode the spatial relationships for the interaction.
% %
% %As shown in the experiments, augmenting the appearance features with spatial features significantly improves the interaction recognition accuracy. 

% %While we adopt the same representation for capturing the relative spatial relationship between the detected human and object, the use of the spatial features differs significantly from~\cite{Chao-WACV-HOI}.
% %
% %Unlike predicting interactions using spatial features alone~\cite{Chao-WACV-HOI}, the purpose of our spatial feature is to augment the appearance features of human, object, and contextual region so that the network can learn to reject plausible but spatially incompatible interactions.

==> table/VCOCO_ablation_augmentation.tex <==
\begin{table}[t]
\centering
\caption{Ablation on V-COCO \emph{test} about which branch to be augmented.}
\label{tab:vcoco_augmentation}

\vspace{2mm}
\begin{tabular}{cc|c}
\toprule
   $S_1$   &    $S_2$   & $AP_{role}$ \\
\midrule
     -     &      -     &  42.5 \\
\checkmark &      -     &  43.3 \\
     -     & \checkmark &  $\underline{43.2}$ \\
\checkmark & \checkmark & \revised{\tb{44.7}} \\
\bottomrule
\end{tabular}
\end{table}
